Optimizing Binary Decision Diagrams with MaxSAT for classification

The growing interest in explainable artificial intelligence (XAI) for critical decision making motivates the need for interpretable machine learning (ML) models. In fact, due to their structure (especially with small sizes), these models are inherently understandable by humans. Recently, several exact methods for computing such models are proposed to overcome weaknesses of traditional heuristic methods by providing more compact models or better prediction quality. Despite their compressed representation of Boolean functions, Binary decision diagrams (BDDs) did not gain enough interest as other interpretable ML models. In this paper, we first propose SAT-based models for learning optimal BDDs (in terms of the number of features) that classify all input examples. Then, we lift the encoding to a MaxSAT model to learn optimal BDDs in limited depths, that maximize the number of examples correctly classified. Finally, we tackle the fragmentation problem by introducing a method to merge compatible subtrees for the BDDs found via the MaxSAT model. Our empirical study shows clear benefits of the proposed approach in terms of prediction quality and intrepretability (i.e., lighter size) compared to the state-of-the-art approaches.

==> 2-responses_reviewers.tex <==
\appendix
\newpage


\section*{General response}
We would like to thank the reviewers for their constructive feedback.
All minor comments and typos will be fixed in the new version. 
An additional typo is to replace the ``\textbf{set} $\{ x_1, \ldots x_n \}$'' by the ``\textbf{sequence} $(x_1, \ldots x_n )$'' in Section 2, \textbf{Binary Decision Diagrams}, second line.

%Before responding to each reviewer, we correct two writing typos in the section ``\textbf{Technical Background}''.
%\begin{enumerate}
%    \item In section ``Classification'', the dataset should be denoted as  $\trainset =\{\atraindataind{1}, \dots, \atraindataind{\nbtraindata}\}$. 
%    Thanks to Reviewer 4.
%    \item In section ``Binary Decision Diagrams'', the word ``\textbf{set}'' in the second sentence should be changed as ``\textbf{sequence}''.
%\end{enumerate}

\section*{Response to Reviewer 1}
%We respond by following the same order as the questions given by Reviewer 1.

 \noindent
 We would like first to comment on the weak points

 \begin{itemize} 
     \item \Bdd{}s are compact representations of Boolean functions. A motivating example (in particular regarding interpretability) can be added.
     \item The current model does not support such hype-parameter, however, it could be extended by constraining the number of nodes via new variables and constraints. 
     \item The different running times are mentioned in the appendix except those for ODT and OODG. 
     
 \end{itemize}
%\def\mo#1{\textbf{#1}}
\noindent
{Answers to the questions:}

\begin{enumerate}
    \item %
    Yes, thanks to the (partial) MaxSAT framework, sample-weights can easily be handled by changing the weights of related soft clauses.
    %We also refer Reviewer 1 to the answer of question 4.
    This is also related to the answer of question 4.
    
    \item %We refer Reviewer 1 to the definition of ``\textit{beads}'' in the third paragraph of section ``Binary Decision Diagrams''. 
    %$\{00, 11\}$ are not \textit{beads} as they both have the form $\alpha\alpha$, when $\alpha$ is `0' and `1'.
    A bead, by definition, does not have the form $\alpha \alpha$ therefore $\{00\}$ and $\{11\}$ are not {beads}. \\
    % The beads of the example are $00010111$, $0111$, $0001$, and $01$..  \\
    The typo that we mentioned in the general response (\textit{sequence} instead of \textit{set}), makes [$x_1, x_2, x_3$] an \textit{ordered sequence}. 
    Therefore, $x_2$ cannot be a child of $x_3$. 
    The construction of the \Bdd{} is done using Proposition 1 and the sequence. 
    
    \item 
    %No, as we assume all binary decision diagrams constructed in this paper are ``\textit{reduced} \& \textit{ordered}''.
    %We also refer Reviewer 1 to the answer of question 5.
    We did not consider \Bdd{}s without the properties \textit{reduced} and \textit{ordered} as they are highly useful and used in the literature [Knuth 2009, Section 7.1.4]. %This point is related to the answer of question 5. 
    For instance, a non \textit{reduced} \Bdd{}   potentially has redundant nodes/branches. 
    
    \item %We did not use ``Partial Weighted MaxSAT'' as the datasets we used contain identical examples and are consistent.
    %However, our formulation is flexible to weighted MaxSAT.
    Yes, such preferences can easily be translated into weights then associated to soft clauses.
%    Please refer to the answer of question 1. 
    %Our formulation is not amenable to negatively classified samples, 
    %it could be interesting if our formulation applied in incremental learning.
    %\med{The presence of negative weights can easily be handled as follows: take $m$ as the minimum of all weights, then update every weight by adding $m$.}
    % Hao: It is not negative weights for example, the question want to know is that possible to add higher weight when wrongly classified, similar idea as Boosting
    
    \item The ``\textit{ordered}''  property is preserved by the definition of the variable set $a_r^i$ to find an ordered sequence of features with constraints 1 and 2.
    
    The (Max)SAT model does not enforce the ``reduced'' property. 
    [Knuth 2009, Section 7.1.4] showed that Proposition 1 guarantees the ``reduced'' property. 
    %The ``reduced''property is
    We therefore apply Proposition 1 on the feature ordering and the truth table decided by the (Max)SAT solver.  We will clarify this in the paper. 
%    We refer Reviewer 1 to \textit{Proposition 1}.
    
    \item The complexity of merging compatible subtrees is $O(k^2)$, where $k$ is the number of subtrees, from~\cite{DBLP:conf/ijcai/KohaviL95}.
    In practice, this process just takes about few seconds. 
    
    \item 
        \begin{itemize}
            \item Yes, we have tried the experiments with higher depth until 9. 
            The testing accuracy of ODT and OODG gets closer to those found \MaxSat\ model. %Overall the testing accuracy does not change much. 
            % \med{TODO : this is not a response to the question}
            %However, the difference between average testing accuracy of \MaxSAT\ with different biases do not vary a lot (less than $5\%$) \med{How about the others?}.
            
            \item
            The average test accuracy of the three MaxSAT-BDD does improve with the growth of maximum depth as shown in Figure 5. 
            % \med{Is this the case with the training accuracy?}
            % Hao: Yes, check the left one in Figure 5
            % \med{always?}
        \end{itemize}
        
    \item Yes, scalabity is an important research direction to investigate. 
    Our heuristic approach is a first step towards this concern and should be further explored. Incremental learning can be helpful in this context.  %to consider in the future work (perhaps on top of our heuristic approach). 
    
    %Combing both is indeed an interesting future research to investigate. 
    
    \item We choose all (and only) the features in the tree constructed by \cart{}.
    %as the candidate features for MaxSAT-BDD.
    The numbers are given in column $\mathbf{F\_d}$ of Table 6 in the appendix.% gives their number.
    \end{enumerate}
    

\section*{Response to Reviewer 2}

Answers to the specific questions:

\begin{enumerate}
    \item Q1:
    % \med{We should answer by saying: minimize BDD is blabla whereas minimizing features is blabla. }
    The number of features is a metric to minimize the \Bdd{}.
    The latter can include other metrics, such as the number of nodes, the classification error, etc.  
    %As \Bdd{}s are assumed as \textit{ordered} and \textit{reduced}, this metric is equal to the maximum depth.
    \item Q2: No, we did not try other encodings.
    Sinz's encoding is standard, easy to use, and did not show any issue in practice. 
    It would be indeed interesting to try others. 
    \item Q3: 
    It is hard to find an explanation.
    % However, this phenomenon at least shows that 
    The only insight we can make is that 
    the solutions are not sensitive to these biases. 
    % \med{
%    perhaps the biases are similar in most cases. %}
    %We know at least that the MaxSAT solutions are robust against such biased. 
    \end{enumerate}
    
   %     \item \textbf{Insights for no substantial difference between different biases chosen for \MaxSat-\Bdd{}}: 
%    We did not make some theoretical analyse to explain this phenomenon, as the initial motivation of the post-processing is to solve the \textit{fragmentation} problem.
 %   However, somehow, this phenomenon indicates that the model \Bdd{} is quite robust with the biases chosen.
%\newline


\noindent
The following are responses to the different comments. 
    %It is easy and quit standard to use  used 
    \begin{itemize}

 
    \item %\textbf{Doubts in motivation}: 
    % \med{This part is not clear and needs discussion. Is this question 1? comment 1? is miniming BDD more general? When did we talk about minimizing a BDD? 
   % 
%    \med{This answer is ambiguous and doesn't answer the question}
%    There could be different metrics to minimize for optimizing BDD, for example, number of nodes, maximum depth, etc.
%    In this paper, we choose the metric of minimizing the number of different features.
    As \Bdd{}s are assumed to be \textit{ordered} and \textit{reduced}, the number of different features is equal to the maximum depth (which is an important metric for the topology). 
    %Therefore minimizing the number of features is different from minimizing the number of nodes. 
% \--> No need for this   
    Contrarily to ~\cite{DBLP:conf/date/CabodiCI0PP21}, the objective of our MaxSAT model of \Bdd{} is to find the \Bdd{} in limited depths that maximizes the number of examples correctly classified.
    % \med{How about comparing the SAT encoding of our with them?}
    % }
    
    \item {On the comparison with ~\cite{DBLP:conf/date/CabodiCI0PP21}}:
    The \Bdd{} found by~\cite{DBLP:conf/date/CabodiCI0PP21} could be small in size, however deep.
    Given a fixed size, one can construct \Bdd{}s with a big difference in depth, making a fair comparison between the two approaches difficult.
    %Given a fixed size, one can construct \Bdd{}s with a big difference in depth. Therefore, making a fair comparison between the two approaches is difficult.
    

\item We can add a short discussion regarding the scalability of BDD1 vs BDD2.
%\item 

%    \item \textbf{Why minimizing the number of features is better?}:
%    In fact, they are two different metrics, 
%    \med{we did not claim which one is better? --> how about interpretability}.
    

    
    \item Loandra is still a state of the art solver. In addition, we used it for a fair comparison with [Hu et al. 2020]. Using alternative MaxSAT solvers is possible. 
%    It is still an efficient incomplete MaxSAT solver.
%    It is also free to use other solvers.
    
    \item %\textbf{How $5$ datasets are selected in Figure 5}:
    In Figure 5, we use $15$ different datasets 
    % (\med{out of 16 but why not all?}) 
    with $5$ different depths. This is mentioned in the caption of Figure 5 well as section ``{Comparison with Existing Heuristic Approaches}''.
    
    % We refer Reviewer 2 to the caption of Figure 5 and the last paragraph of section ``Comparison with Existing Heuristic Approaches''.
    
    %\item \textbf{No definition of \MaxSat-\DT{}}: 
    %We will add the sentence that notes \MaxSat-\DT{} is the \MaxSat model of Decision Tree in~\cite{DBLP:conf/ijcai/Hu0HH20} in further version.
    
%    \item \textbf{Results in supplemental material}: 
 %   As the limited pages and the readability of the paper, we consider it could be difficult to put all results in the main paper.
\end{itemize}



\section*{Response to Reviewer 3}

\begin{enumerate}
    \item Table 6 in the appendix reports the running time. 
    
  %  \item \textbf{Why not accuracy are not improved with the increase of depth}:
  %  As we used incomplete MaxSAT solver within same limited time, the encoding size increase with the increase of depth. 
  %  Therefore, if \textit{optimality} is not reported, this phenomenon is possible.
  \item %The different calls to the solver are independent. 
  When the depth grows, the encoding size as well as the search space gets bigger. Hence the solver ``struggels'' to explore the search space.
    
\end{enumerate}

\section*{Response to Reviewer 4}

Extensions to non-integer features is an interesting future work. One can for instance binarize the features based on some thresholds.


==> tables/Ex2-Var-Sat-model.tex <==
\scalebox{0.8}{
        \begin{tabular}{|cc||c|}
            \hline
            $\avarind{1}$ & $\avarind{2}$ & \\\hline
            $0$ & $0$ & $\adecisionind{1}$ \\\hline
            $0$ & $1$ & $\adecisionind{2}$ \\\hline
            $1$ & $0$ & $\adecisionind{3}$ \\\hline
            $1$ & $1$ & $\adecisionind{4}$ \\\hline
        \end{tabular}
        }
        \caption{\footnotesize{Truth table for a \texttt{BDD} with a depth $\depth=2$}}
        \label{tab:Bdd-variables}

==> tables/Exp3_smaller.tex <==
\begin{table}[!h]
    \centering
    % \resizebox{.9}{!}{
    \renewcommand{\arraystretch}{0.75}
    \setlength{\tabcolsep}{1.2pt}
    \scriptsize{}
    \begin{tabular}{|c|c||c|c|c|c||c|c|c|c||}
    \hline
    \multirow{2}{*}{\scriptsize{\textbf{Datasets}}} & 
    \multirow{2}{*}{\scriptsize{\textbf{\depth{}}}} &
    \multicolumn{4}{c||}{\scriptsize{\textbf{MaxSAT BDD-C}}} & 
    \multicolumn{4}{c||}{\scriptsize{\textbf{MaxSAT-DT}}} \\
    \cline{3-10} 
            & &
            \cellcolor{cyan!15}\textbf{Train} &
            \cellcolor{orange!15}\textbf{Test} &
            \cellcolor{green!15}\textbf{Size} &
            \cellcolor{yellow!30}\textbf{E\_Size} 
            & \cellcolor{cyan!15}\textbf{Train} &
            \cellcolor{orange!15}\textbf{Test} & 
            \cellcolor{green!15}\textbf{Size} &
            \cellcolor{yellow!30}\textbf{E\_Size}\\ 
    \hline
    
    \multirow{4}{*}{\shortstack[1]{anneal\\(812/89)}}
 & 2 & 82.92 & \cellcolor{red!50}82.19 & \cellcolor{red!50}5 & \cellcolor{red!50}24.09 & \cellcolor{red!50}83.18 & 82.14 & 6.84 & 52.72\\
 & 3 & 84 & 83.55 & \cellcolor{red!50}7 & \cellcolor{red!50}37.21 & \cellcolor{red!50}85.07 & \cellcolor{red!50}84.61 & 12.60 & 126.18\\
 & 4 & 84.58 & 83.84 & \cellcolor{red!50}9.4 & \cellcolor{red!50}52.06 & \cellcolor{red!50}86.04 & \cellcolor{red!50}84.73 & 18.60 & 315.45\\
 & 5 & 85.33 & 83.92 & \cellcolor{red!50}11.72 & \cellcolor{red!50}71.08 & \cellcolor{red!50}86.48 & \cellcolor{red!50}84.97 & 23.88 & 865.26\\
\hline

\multirow{4}{*}{\shortstack[1]{audiology\\(216/146)}}
 & 2 & 94.91 & \cellcolor{red!50}94.92 & \cellcolor{red!50}4 & \cellcolor{red!50}10.59 & \cellcolor{red!50}95.49 & \cellcolor{red!50}94.92 & 7 & 31.35\\
 & 3 & 96.78 & \cellcolor{red!50}95.84 & \cellcolor{red!50}5.04 & \cellcolor{red!50}16.41 & \cellcolor{red!50}97.85 & 95.56 & 11.64 & 88.75\\
 & 4 & 97.73 & \cellcolor{red!50}95.56 & \cellcolor{red!50}6.96 & \cellcolor{red!50}22.56 & \cellcolor{red!50}99.51 & 94.54 & 19.08 & 272.15\\
 & 5 & 98.40 & \cellcolor{red!50}94.44 & \cellcolor{red!50}9.88 & \cellcolor{red!50}29.82 & \cellcolor{red!50}99.95 & 94.26 & 27.48 & 915.29\\
\hline

\multirow{4}{*}{\shortstack[1]{australian\\(653/124)}}
 & 2 & 86.70 & \cellcolor{red!50}85.94 & \cellcolor{red!50}4.72 & \cellcolor{red!50}26.79 & \cellcolor{red!50}86.93 & 85.33 & 6.68 & 59.65\\
 & 3 & 87.45 & \cellcolor{red!50}84.81 & \cellcolor{red!50}5.32 & \cellcolor{red!50}41.15 & \cellcolor{red!50}88.11 & 84.72 & 13.08 & 146.15\\
 & 4 & 88.45 & \cellcolor{red!50}86.03 & \cellcolor{red!50}7.4 & \cellcolor{red!50}56.85 & \cellcolor{red!50}88.74 & 85.15 & 17.48 & 377.62\\
 & 5 & \cellcolor{red!50}89.36 & \cellcolor{red!50}85.91 & \cellcolor{red!50}10.44 & \cellcolor{red!50}75.9 & 89.22 & 84.78 & 22.20 & 1076.35\\
\hline

\multirow{4}{*}{\shortstack[1]{cancer\\(683/89)}}
 & 2 & 93.88 & 93.59 & \cellcolor{red!50}4 & \cellcolor{red!50}20.29 & \cellcolor{red!50}94.91 & \cellcolor{red!50}94.2 & 7 & 45.56\\
 & 3 & 95.02 & 93.91 & \cellcolor{red!50}5.84 & \cellcolor{red!50}31.37 & \cellcolor{red!50}96.61 & \cellcolor{red!50}94.79 & 15 & 110.85\\
 & 4 & 96.06 & \cellcolor{red!50}95.49 & \cellcolor{red!50}7.96 & \cellcolor{red!50}43.89 & \cellcolor{red!50}97.34 & 94.20 & 21.08 & 283.77\\
 & 5 & 95.94 & 93.74 & \cellcolor{red!50}10.68 & \cellcolor{red!50}59.91 & \cellcolor{red!50}97.97 & \cellcolor{red!50}94.29 & 29.24 & 800.89\\
\hline

\multirow{4}{*}{\shortstack[1]{car\\(1728/21)}}
 & 2 & \cellcolor{red!50}85.53 & \cellcolor{red!50}85.53 & \cellcolor{red!50}4 & \cellcolor{red!50}13.32 & \cellcolor{red!50}85.53 & \cellcolor{red!50}85.53 & 6.84 & 32.01\\
 & 3 & 88.40 & 87.41 & \cellcolor{red!50}5.08 & \cellcolor{red!50}21.95 & \cellcolor{red!50}89.25 & \cellcolor{red!50}87.45 & 12.68 & 71.83\\
 & 4 & 89.84 & 88.54 & \cellcolor{red!50}6.84 & \cellcolor{red!50}34.44 & \cellcolor{red!50}91.62 & \cellcolor{red!50}89.68 & 20.36 & 162.46\\
 & 5 & 91.13 & 89.91 & \cellcolor{red!50}9.6 & \cellcolor{red!50}55.79 & \cellcolor{red!50}93.76 & \cellcolor{red!50}92.7 & 29.32 & 389.68\\
\hline

\multirow{4}{*}{\shortstack[1]{cleveland\\(296/95)}}
 & 2 & 79.04 & 72.57 & \cellcolor{red!50}4 & \cellcolor{red!50}9.48 & \cellcolor{red!50}80.79 & \cellcolor{red!50}72.7 & 7 & 25.57\\
 & 3 & 85.07 & \cellcolor{red!50}83.37 & \cellcolor{red!50}6 & \cellcolor{red!50}14.73 & \cellcolor{red!50}85.83 & 76.75 & 12.92 & 68.93\\
 & 4 & 86.32 & \cellcolor{red!50}79.46 & \cellcolor{red!50}7.84 & \cellcolor{red!50}20.55 & \cellcolor{red!50}86.71 & 76.41 & 17.80 & 200.76\\
 & 5 & \cellcolor{red!50}88.65 & \cellcolor{red!50}78.72 & \cellcolor{red!50}13.08 & \cellcolor{red!50}27.89 & 87.26 & 74.45 & 23.96 & 646.75\\
\hline

\multirow{4}{*}{\shortstack[1]{hypothyroid\\(3247/86)}}
 & 2 & \cellcolor{red!50}97.84 & \cellcolor{red!50}97.84 & \cellcolor{red!50}4 & \cellcolor{red!50}92.65 & \cellcolor{red!50}97.84 & \cellcolor{red!50}97.84 & 5.96 & 182.20\\
 & 3 & 98.09 & \cellcolor{red!50}98.04 & \cellcolor{red!50}5.12 & \cellcolor{red!50}142.78 & \cellcolor{red!50}98.14 & 97.82 & 9.72 & 402.98\\
 & 4 & 98.27 & \cellcolor{red!50}98.13 & \cellcolor{red!50}6.72 & \cellcolor{red!50}200.09 & \cellcolor{red!50}98.38 & 98.01 & 15.40 & 885.51\\
 & 5 & 98.30 & \cellcolor{red!50}98.05 & \cellcolor{red!50}9.28 & \cellcolor{red!50}274.03 & \cellcolor{red!50}98.46 & 97.99 & 20.44 & 2016.31\\
\hline

\multirow{4}{*}{\shortstack[1]{kr-vs-kp\\(3196/73)}}
 & 2 & 77.83 & 77.01 & \cellcolor{red!50}4 & \cellcolor{red!50}77.88 & \cellcolor{red!50}86.92 & \cellcolor{red!50}86.92 & 7 & 155.09\\
 & 3 & 90.43 & 90.43 & \cellcolor{red!50}5.28 & \cellcolor{red!50}120.54 & \cellcolor{red!50}93.67 & \cellcolor{red!50}93.67 & 12.36 & 342.99\\
 & 4 & 94.09 & 94.09 & \cellcolor{red!50}7.56 & \cellcolor{red!50}170.28 & \cellcolor{red!50}94.37 & \cellcolor{red!50}94.14 & 17.40 & 753.78\\
 & 5 & 94.34 & 94.18 & \cellcolor{red!50}9.52 & \cellcolor{red!50}236.39 & \cellcolor{red!50}94.84 & \cellcolor{red!50}94.66 & 25.40 & 1717.14\\
\hline

\multirow{4}{*}{\shortstack[1]{lymph\\(148/68)}}
 & 2 & 84.46 & \cellcolor{red!50}83.23 & \cellcolor{red!50}4 & \cellcolor{red!50}3.5 & \cellcolor{red!50}86.01 & 79.27 & 7 & 12.33\\
 & 3 & 86.76 & 78.35 & \cellcolor{red!50}5.92 & \cellcolor{red!50}5.55 & \cellcolor{red!50}91.96 & \cellcolor{red!50}80.68 & 14.68 & 36.65\\
 & 4 & 90.54 & \cellcolor{red!50}82.4 & \cellcolor{red!50}8.72 & \cellcolor{red!50}7.86 & \cellcolor{red!50}94.56 & 78.47 & 20.28 & 117.94\\
 & 5 & 93.51 & \cellcolor{red!50}83.6 & \cellcolor{red!50}13.52 & \cellcolor{red!50}10.94 & \cellcolor{red!50}97.06 & 82.86 & 26.92 & 413.09\\
\hline

\multirow{4}{*}{\shortstack[1]{mushroom\\(8124/112)}}
 & 2 & 95.13 & 95.13 & \cellcolor{red!50}4 & \cellcolor{red!50}299.19 & \cellcolor{red!50}96.9 & \cellcolor{red!50}96.9 & 7 & 565.27\\
 & 3 & 97.74 & 97.77 & \cellcolor{red!50}6.8 & \cellcolor{red!50}458.1 & \cellcolor{red!50}99.9 & \cellcolor{red!50}99.9 & 13.72 & 1227.18\\
 & 4 & 98.78 & 98.74 & \cellcolor{red!50}9 & \cellcolor{red!50}635.09 & \cellcolor{red!50}100 & \cellcolor{red!50}100 & 19.96 & 2603.94\\
 & 5 & 98.63 & 98.57 & \cellcolor{red!50}11.32 & \cellcolor{red!50}853.68 & \cellcolor{red!50}100 & \cellcolor{red!50}100 & 23.40 & 5571.14\\
\hline

\multirow{4}{*}{\shortstack[1]{tumor\\(336/31)}}
 & 2 & 82.80 & \cellcolor{red!50}81.6 & \cellcolor{red!50}4 & \cellcolor{red!50}3.72 & \cellcolor{red!50}82.92 & 81.01 & 6.76 & 10.46\\
 & 3 & 83.84 & 80.43 & \cellcolor{red!50}5.3 & \cellcolor{red!50}6.02 & \cellcolor{red!50}86.25 & \cellcolor{red!50}83.56 & 13.72 & 27.24\\
 & 4 & 85.52 & 82.49 & \cellcolor{red!50}8.64 & \cellcolor{red!50}9.04 & \cellcolor{red!50}87.96 & \cellcolor{red!50}82.79 & 21.40 & 76.40\\
 & 5 & 87.51 & \cellcolor{red!50}85.83 & \cellcolor{red!50}13.32 & \cellcolor{red!50}13.79 & \cellcolor{red!50}90.09 & 79.34 & 47.80 & 239.09\\
\hline

\multirow{4}{*}{\shortstack[1]{soybean\\(630/50)}}
 & 2 & 90.48 & 90.48 & \cellcolor{red!50}4 & \cellcolor{red!50}10.79 & \cellcolor{red!50}91.27 & \cellcolor{red!50}91.27 & 7 & 25.55\\
 & 3 & 91.39 & 90.41 & \cellcolor{red!50}6.52 & \cellcolor{red!50}16.99 & \cellcolor{red!50}95.45 & \cellcolor{red!50}94.7 & 15 & 62.30\\
 & 4 & 93.24 & 93.21 & \cellcolor{red!50}9.04 & \cellcolor{red!50}24.54 & \cellcolor{red!50}97.28 & \cellcolor{red!50}95.81 & 22.20 & 160.18\\
 & 5 & 94.31 & 92.95 & \cellcolor{red!50}11.92 & \cellcolor{red!50}35.34 & \cellcolor{red!50}98.05 & \cellcolor{red!50}95.21 & 40.68 & 455.33\\
\hline

\multirow{4}{*}{\shortstack[1]{splice-1\\(3190/287)}}
 & 2 & 84.04 & \cellcolor{red!50}84.04 & \cellcolor{red!50}4 & \cellcolor{red!50}296.61 & \cellcolor{red!50}84.23 & 83.12 & 6.92 & 555.22\\
 & 3 & 87.25 & 86.94 & \cellcolor{red!50}5.44 & \cellcolor{red!50}449.04 & \cellcolor{red!50}87.62 & \cellcolor{red!50}87.25 & 11.32 & 1231.59\\
 & 4 & \cellcolor{red!50}88.3 & \cellcolor{red!50}88.04 & \cellcolor{red!50}7.24 & \cellcolor{red!50}608.3 & 87.25 & 86.42 & 16.60 & 2717.90\\
 & 5 & 71.99 & 70.53 & \cellcolor{red!50}10.28 & \cellcolor{red!50}783.9 & \cellcolor{red!50}76.85 & \cellcolor{red!50}75.82 & 22.10 & 6226.75\\
\hline

\multirow{4}{*}{\shortstack[1]{tic-tac-toe\\(958/27)}}
 & 2 & 71.05 & \cellcolor{red!50}68.35 & \cellcolor{red!50}4 & \cellcolor{red!50}9.25 & \cellcolor{red!50}71.1 & 67.49 & 5.96 & 22.31\\
 & 3 & 74.91 & 72.36 & \cellcolor{red!50}6.16 & \cellcolor{red!50}15.01 & \cellcolor{red!50}77.2 & \cellcolor{red!50}73.3 & 11.48 & 51.98\\
 & 4 & 76.87 & 74.22 & \cellcolor{red!50}8.84 & \cellcolor{red!50}22.88 & \cellcolor{red!50}82.46 & \cellcolor{red!50}78.7 & 20.60 & 125.10\\
 & 5 & 81.86 & \cellcolor{red!50}80.31 & \cellcolor{red!50}13.88 & \cellcolor{red!50}35.67 & \cellcolor{red!50}83.11 & 79.54 & 28.36 & 328.33\\
\hline

\multirow{4}{*}{\shortstack[1]{vote\\(435/48)}}
 & 2 & 95.68 & \cellcolor{red!50}95.22 & \cellcolor{red!50}3.76 & \cellcolor{red!50}7.2 & \cellcolor{red!50}96.21 & 95.03 & 7 & 18.33\\
 & 3 & 96.69 & \cellcolor{red!50}94.57 & \cellcolor{red!50}5.56 & \cellcolor{red!50}11.38 & \cellcolor{red!50}97.38 & 93.84 & 13.88 & 46.55\\
 & 4 & 97.40 & 94.39 & \cellcolor{red!50}8.16 & \cellcolor{red!50}16.49 & \cellcolor{red!50}98.66 & \cellcolor{red!50}94.53 & 21.56 & 126.45\\
 & 5 & 98.21 & \cellcolor{red!50}94.57 & \cellcolor{red!50}12.4 & \cellcolor{red!50}23.83 & \cellcolor{red!50}99.47 & 93.84 & 30.52 & 381.95\\
\hline

    \end{tabular}
    \caption{\label{tab:exp3_maxsatbdd_maxsatdt_all_small}
    \footnotesize{Comparison between \MaxSat\ model for \Bdd{}s and \MaxSat\ model for decision trees.}
    }
\end{table}
